Vision Transformer Adapter for Dense Predictions

This work investigates a simple yet powerful dense prediction task adapter for Vision Transformer (ViT). Unlike recently advanced variants that incorporate vision-specific inductive biases into their architectures, the plain ViT suffers inferior performance on dense predictions due to weak prior assumptions. To address this issue, we propose the ViT-Adapter, which allows plain ViT to achieve comparable performance to vision-specific transformers. Specifically, the backbone in our framework is a plain ViT that can learn powerful representations from large-scale multi-modal data. When transferring to downstream tasks, a pre-training-free adapter is used to introduce the image-related inductive biases into the model, making it suitable for these tasks. We verify ViT-Adapter on multiple dense prediction tasks, including object detection, instance segmentation, and semantic segmentation. Notably, without using extra detection data, our ViT-Adapter-L yields state-of-the-art 60.9 box AP and 53.0 mask AP on COCO test-dev. We hope that the ViT-Adapter could serve as an alternative for vision-specific transformers and facilitate future research. The code and models will be released at https://github.com/czczup/ViT-Adapter.

==> table/efficiency.tex <==
\begin{table}[t]\small
	\centering
	\renewcommand\arraystretch{1.0}
    \setlength\tabcolsep{0.57mm}
    \begin{tabular}{l|cccc|ccc|cc}
        \toprule
        Method & Segmentor & Pre-train & \#Param & FLOPs & Train Time & Train Mem. & FPS & mIoU$_{\rm ss}$ & mIoU$_{\rm ms}$ \\
	    \midrule
        ViT-B & SETR-PUP   & IN-1K     & 98M     & 170G  & 0.16s/iter & 9.5G & 30.3  & 46.3 & 47.3  \\ 
        ViT-B & Semantic FPN     & IN-1K     & 98M     & 147G  & 0.15s/iter & 5.6G & 29.7  & 46.4 & 47.6  \\ 
        \rowcolor{gray!20} 
        ViT-Adapter-B & Semantic FPN & IN-1K & 105M    & 183G  & 0.16s/iter & 7.5G & 26.7  & \textbf{47.9} & \textbf{48.9}  \\
        \midrule
        ViT-L & SETR-PUP   & IN-22K     & 318M    & 425G  & 0.25s/iter & 16.8G & 14.0  & 48.6 & 50.1  \\ 
        ViT-L & Semantic FPN     & IN-22K     & 321M     & 414G  & 0.21s/iter & 14.1G & 15.5  & 51.5 & 52.0  \\ 
        \rowcolor{gray!10} 
        ViT-Adapter-L$_{\rm light}$ & Semantic FPN & IN-22K & 324M & 445G  & 0.23s/iter & 15.2G & 13.5 & 52.7 & 53.5  \\
        \rowcolor{gray!20} 
        ViT-Adapter-L & Semantic FPN & IN-22K & 332M    & 473G  & 0.25s/iter & 16.0G & 12.9  & \textbf{52.9} & \textbf{53.7}  \\
	    \bottomrule
    \end{tabular}
    \caption{\textbf{Efficiency analysis of ViT-Adapter for semantic segmentation.} 
    We equip our ViT-Adapter models with Semantic FPN~\citep{kirillov2019panoptic} for segmentation and compared them with the representative ViT-based method SETR~\citep{zheng2021rethinking}.
    We use a single A100 GPU and FP16 mode to benchmark these models.
    The training time and training memory are measured with a batch size of 2, and the FPS is tested with a batch size of 1. 
    The FLOPs is calculated with 512$\times$512 inputs.
    % IN-1K/-22K is short for ImageNet-1K/-22K.
    $\rm {light}$: We build a lightweight model by reducing the width of the adapter.
    }
    \label{tab:efficiency}
\end{table}
% \vspace{-1em}
\begin{table}[t]\small
	\centering
	\renewcommand\arraystretch{1.0}
    \setlength\tabcolsep{1.32mm}
    \begin{tabular}{l|cccc|ccc|cc}
        \toprule
        Method & Detector & Pre-train & \#Param & FLOPs & Train Time & Train Mem. & FPS & AP${\rm ^b}$ & AP${\rm ^m}$ \\
	    \midrule
        ViT-B    & Mask R-CNN & IN-1K & 114M & 692G  & 0.25s/iter & 18.3G & 17.4  & 45.8 & 41.3  \\ 
        ViTDet-B & Mask R-CNN & IN-1K & 121M & 747G  & 0.25s/iter & 18.2G & 17.1  & 46.3 & 41.6  \\ 
        \rowcolor{gray!20} 
        ViT-Adapter-B & Mask R-CNN & IN-1K & 120M & 832G  & 0.32s/iter & 21.7G & 13.5  & \textbf{49.6} & \textbf{43.6}  \\
        \midrule
        ViT-L    & Mask R-CNN & IN-22K & 337M & 1.7T  & 0.44s/iter & 33.9G & 9.2 & 48.3 & 43.4  \\ 
        ViTDet-L & Mask R-CNN & IN-22K & 350M & 1.9T  & 0.45s/iter & 33.8G & 9.0  & 49.1 & 44.0  \\ 
        \rowcolor{gray!20} 
        ViT-Adapter-L & Mask R-CNN & IN-22K & 347M & 1.9T  & 0.52s/iter & 37.6G & 7.8  & \textbf{52.1} & \textbf{46.0}  \\
	    \bottomrule
    \end{tabular}
    \caption{\textbf{Efficiency analysis of ViT-Adapter for object detection.} 
    We benchmark all ViT-based methods with Mask R-CNN 3$\times$ schedule. 
    % We use a single A100 GPU with FP16 mode to benchmark these models.
    % The training overhead and inference FPS are measured using the same strategy as discribed in Table~\ref{tab:efficiency}. 
    The training time/memory are measured with a batch size of 2, and the FPS is tested with a batch size of 1. 
    The FLOPs is calculated with 1280$\times$800 inputs.
    }
    \vspace{-1em}
    \label{tab:efficiency_det}
\end{table}

==> table/pretrain_source.tex <==

\begin{table}[t]\small
	\centering
	\renewcommand\arraystretch{1.0}
    \setlength\tabcolsep{1.6mm}
    \begin{tabular}{l|c|ccc|c}
        \toprule
        \multirow{2}{*}{Pre-training Method} & \multirow{2}{*}{Year} & \multicolumn{3}{c|}{Pre-training Type} & \multirow{2}{*}{Dataset}\\
         & & Supervised & Self-supervised & Multi-Modal & \\
        \midrule
        DeiT~\citep{touvron2021training} & 2021 & \checkmark & & &ImageNet-1K\\
        AugReg~\citep{steiner2021train} & 2021 & \checkmark & & &ImageNet-22K\\
        \rowcolor{yellow!15} 
        Uni-Perceiver~\citep{zhu2021uni} & 2021 & \checkmark & & \checkmark &  Multi-Modal Data\\
        MAE~\citep{he2021masked} & 2021 & &\checkmark & & ImageNet-1K\\
        BEiT~\citep{bao2021beit} & 2021 & &\checkmark & & ImageNet-22K\\
        BEiTv2~\citep{peng2022beitv2} & 2022 & &\checkmark & & ImageNet-22K\\
        \rowcolor{yellow!15} 
        BEiTv3~\citep{wang2022beit3} & 2022 & &\checkmark & \checkmark& Multi-Modal Data\\
	    \bottomrule
    \end{tabular}
    \caption{\textbf{Supported pre-training techniques.} 
    Since our paradigm retains the flexibility of the plain ViT, it can utilize various readily available pre-trained weights. 
    }
    \label{tab:pretrain_source}
\end{table}

==> table/result_ade_fpn.tex <==
\begin{table}[t]
	\centering
    \setlength\tabcolsep{8pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}[t]{l|ccc}
        \Xhline{1.0pt}
        \multirow{2}{*}{Method} & \multicolumn{3}{c}{Semantic FPN 80K}\\
         &   \#Param(M) & FLOPs(G) & mIoU(\%) \\ 
         
        \Xhline{1.0pt}
        
        \rowcolor{gray!5} 
        ViT-T$^*$~\cite{li2021benchmarking} & - & - & - \\
        \rowcolor{gray!13}
        ViT-T+DA$_a$~(ours) & - & - & - \\
        \rowcolor{gray!25}
        ViT-T+DA$_b$~(ours) & - & - & - \\
        
        \Xhline{1.0pt}
        PVT-Small \cite{wang2021pyramid} & - & - & - \\
        Swin-T \cite{liu2021swin} & - & - & - \\
        \rowcolor{gray!5} 
        ViT-S$^*$~\cite{li2021benchmarking} & - & - & - \\
        \rowcolor{gray!13}
        ViT-S+DA$_a$~(ours) & - & - & - \\
        \rowcolor{gray!25}
        ViT-S+DA$_b$~(ours) & - & - & - \\
        
        \Xhline{1.0pt}
        \rowcolor{gray!5} 
        PVT-Medium \cite{wang2021pyramid} & - & - & - \\
        Swin-S \cite{liu2021swin} & - & - & - \\
        
        ViT-B$^*$~\cite{li2021benchmarking} & - & - & - \\
        \rowcolor{gray!13}
        ViT-B+DA$_a$~(ours) & - & - & - \\
        \rowcolor{gray!25}
        ViT-B+DA$_b$~(ours) & - & - & - \\
        \Xhline{1.0pt}
    \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\textbf{Semantic segmentation with semantic FPN on ADE20K.} The FLOPs are measured at resolution 512$\times$512.
    }
    \vspace{-0.3cm}
    \label{tab:results_ade_fpn}
\end{table}

==> table/result_ade_upernet.tex <==
\begin{table}[t]
	\centering
    \setlength\tabcolsep{2pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}[t]{l|cccc}
        \Xhline{1.0pt}
        \multirow{2}{*}{Method} & \multicolumn{4}{c}{Upernet 160K}\\
         &  \#Param(M) & FLOPs(G) & mIoU(\%) & MS mIoU(\%) \\ 
        \Xhline{1.0pt}
        Swin-T \cite{liu2021swin} & -  & - & - & - \\
        \rowcolor{gray!5} 
        ViT-T$^*$~\cite{li2021benchmarking} & - & - & - & - \\
        \rowcolor{gray!13}
        ViT-T+DA$_a$~(ours) & - & - & - & - \\
        \rowcolor{gray!25}
        ViT-T+DA$_b$~(ours) & - & - & - & - \\
        \Xhline{1.0pt}
        
        Swin-S \cite{liu2021swin} & - & - & - & - \\
        \rowcolor{gray!5} 
        ViT-S$^*$~\cite{li2021benchmarking} & - & - & - & - \\
        \rowcolor{gray!13}
        ViT-S+DA$_a$~(ours) & - & - & - & - \\
        \rowcolor{gray!25}
        ViT-S+DA$_b$~(ours) & - & - & - & - \\
        
        \Xhline{1.0pt}
        Swin-B \cite{liu2021swin} & - & - & - & - \\
        \rowcolor{gray!5} 
        ViT-B$^*$~\cite{li2021benchmarking} & - & - & - & - \\
        \rowcolor{gray!13}
        ViT-B+DA$_a$~(ours) & - & - & - & - \\
        \rowcolor{gray!25}
        ViT-B+DA$_b$~(ours) & - & - & - & - \\
        \Xhline{1.0pt}
    \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\textbf{Semantic segmentation with Upernet on ADE20K.} The FLOPs are measured at resolution $\times$.}
    \vspace{-0.5cm}
    \label{tab:results_ade_upernet}
\end{table}

==> table/result_detection_benchmark.tex <==
\begin{table}[t]\scriptsize
% 	\renewcommand{\arraystretch}{1.1}
    \caption{\textbf{Performance comparisons with upgraded Mask R-CNN with MAE pre-trained weights.}
    ``$*$"~indicates following \cite{li2021benchmarking} to produce multi-scale feature maps with transposed convolutions.
    ``$_{\rm global}$" denotes using global attention in all layers of ViT, otherwise following the settings of \cite{li2021benchmarking}.
    AP$^\text{b}$ and AP$^\text{m}$ represent box AP and mask AP, respectively.
    }
    
    \begin{minipage}{0.35\textwidth}%
        \setlength\tabcolsep{0.3mm}{
        \begin{tabular}{l|ccc|ccc}
            \toprule
            Method & \#Param & FLOPs &FPS & Epoch & $\rm AP^{b}$ & $\rm AP^{m}$ \\
    	    \midrule
            \multirow{3}{*}{ViT-B$^*$ \cite{li2021benchmarking}} & \multirow{3}{*}{116M} & \multirow{3}{*}{853G} & \multirow{3}{*}{5.1} & 25 & 48.1 & 43.2  \\ 
            ~ & ~ & ~& & 50 & 50.1 & 44.6  \\ 
            ~ & ~ & ~& & 100 & 50.3 & 44.9  \\ 
            \midrule
            % \rowcolor{gray!8} 
             &  &  &
             & 25 & 48.9 & 43.6  \\ 
            % \rowcolor{gray!8} 
            \multirow{-2}{*}{ViT-B$^*_{\rm global}$ \cite{li2021benchmarking}} & \multirow{-2}{*}{116M} & \multirow{-2}{*}{1044G} & \multirow{-2}{*}{3.8} & 50 & 50.2 & 44.5  \\ 
            \midrule
            \rowcolor{gray!20} 
            &  & &  & 25 & 50.3 & 44.7  \\
            \rowcolor{gray!20} 
            \multirow{-2}{*}{ViT-Adapter-B (ours)} & \multirow{-2}{*}{122M} & \multirow{-2}{*}{997G} & \multirow{-2}{*}{4.4} & 50 & 50.8 & 45.1  \\
    	    \bottomrule
        \end{tabular}
        }
    \end{minipage}
    \hspace{12.0em}
    \begin{minipage}{0.35\textwidth}%
    \includegraphics[width=1\linewidth]{figure/curve1.pdf}
    \end{minipage}
    
    
    \label{tab:results_detection_benchmark}
\end{table}

==> table/robustness.tex <==

\begin{table}[!t!]\scriptsize
	\centering
% 	\renewcommand{\arraystretch}{1.1}
	\caption{\textbf{Object detection results on COCO-C based on Mask R-CNN.} 
	``$*$"~indicates following \cite{li2021benchmarking} to produce multi-scale feature maps with transposed convolutions.
	$^\bigstar$~indecates using multi-modal pre-trained weights from~\cite{zhu2021uni}.
	The third column is the average results on 16 types of corruption data.
	}
% 	\hspace{-3.2mm}
	\begin{center}
        \resizebox{1.01\linewidth}{!}{
        \hspace{-3.0mm}
        	\setlength{\tabcolsep}{0.2mm}{
                \begin{tabular}{l|c c|cccc|cccc|cccc|cccc}
                \toprule
                \multirow{2}{*}{Method} & \multirow{2}{*}{Clean} &\multirow{2}{*}{Mean} &\multicolumn{4}{c|}{Blur} & \multicolumn{4}{c|}{Noise} & \multicolumn{4}{c|}{Digital} & \multicolumn{4}{c}{Weather} \\
                \cline{4-19}
                &  & & Motion & Defoc & Glass & \multicolumn{1}{c|}{Gauss} & Gauss & Impul & Shot & \multicolumn{1}{c|}{Speck} & Bright & Contr & Satur & \multicolumn{1}{l|}{JPEG} & \multicolumn{1}{l}{Snow} & \multicolumn{1}{l}{Spatt} & \multicolumn{1}{l}{Fog} & \multicolumn{1}{l}{Frost} \\
                \midrule
                % \multicolumn{1}{l|}{PVTv2-B0~\cite{wang2021pvtv2}} & 41.6 &  &  &  &  & &  &  &  & &  &  &  & &  &  &  &  \\
                \multicolumn{1}{l|}{PVTv2-B1~\cite{wang2021pvtv2}} & 44.9 & 35.1 & 31.1 & 30.6 & 23.7 & 33.7 & 33.0 & 31.8 & 33.2 & 36.1 & 43.3 & 42.0 & 42.5 & 30.8 & 32.4 & 40.4 & 42.1 & 34.6 \\
                \multicolumn{1}{l|}{ViT-T$^*$~\cite{li2021benchmarking}} & 40.2 & 30.0 & 26.2 & 26.5 & 22.8 & 31.2 & 27.1 & 24.7 & 27.0 & 30.5 & 38.3 & 33.8 & 37.3 & 29.3 & 25.7 & 35.1 & 35.5 & 29.1 \\
                \rowcolor{gray!20}
                \multicolumn{1}{l|}{ViT-Adapter-T} & \textbf{46.0} & \textbf{35.6} & 32.5 & 32.6 & 26.5 & 35.3 & 31.0 & 30.6 & 31.1 & 35.3 & 44.2 & 42.1 & 43.5 & 33.3 & 31.5 & 41.4 & 42.9 & 35.8 \\
                \midrule
                \multicolumn{1}{l|}{PVTv2-B2~\cite{wang2021pvtv2}} & 47.8 & 37.7 & 34.1 & 31.5 & 27.9 & 33.9 & 36.8 & 37.0 & 37.2 & 40.0 & 46.2 & 42.5 & 40.2 & 34.1 & 35.8 & 44.0 & 43.8 & 38.3 \\
                \multicolumn{1}{l|}{Swin-T~\cite{liu2021swin}} & 46.0 & 35.3 & 31.3 & 32.5 & 23.2 & 35.6 & 32.1 & 31.4 & 32.2 & 35.7 & 44.1 & 41.4 & 43.5 & 32.0 & 30.9 & 41.2 & 42.7 & 34.4 \\
                \multicolumn{1}{l|}{ViT-S$^*$~\cite{li2021benchmarking}} & 44.0 & 34.3 & 31.4 & 30.9 & 26.0 & 33.8 & 31.0 & 29.3 & 31.1 & 34.6 & 42.3 & 38.0 & 41.3 & 35.0 & 30.4 & 39.6 & 39.7 & 33.6 \\
                \rowcolor{gray!20}
                \multicolumn{1}{l|}{ViT-Adapter-S} & \textbf{48.2} & \textbf{37.8} & 34.5 & 34.1 & 28.9 & 37.2 & 33.2 & 33.3 & 33.5 & 37.5 & 46.4 & 43.6 & 45.8 & 37.1 & 34.2 & 43.6 & 44.7 & 37.5 \\
                \midrule
                \multicolumn{1}{l|}{PVTv2-B5~\cite{wang2021pvtv2}} & 48.4 & 38.6 & 33.8 & 34.2 & 28.9 & 32.6 & 38.2 & 38.9 & 38.5 & 41.0 & 46.7 & 38.7 & 46.2 & 37.5 & 36.5 & 44.4 & 43.3 & 38.1 \\
                \multicolumn{1}{l|}{Swin-B~\cite{liu2021swin}} & 48.6 & 37.8 & 33.5 & 34.3 & 25.3 & 37.7 & 35.1 & 34.7 & 35.3 & 38.6 & 46.8 & 43.7 & 46.1 & 35.8 & 33.2 & 43.9 & 45.0 & 36.5 \\
                \multicolumn{1}{l|}{ViT-B$^*$~\cite{li2021benchmarking}} & 45.8 & 36.8 & 32.6 & 33.2 & 27.9 & 36.0 & 34.6 & 33.5 & 34.7 & 37.6 & 44.3 & 41.4 & 43.5 & 36.9 & 33.1 & 41.6 & 42.3 & 35.3 \\
                \rowcolor{gray!20}
                \multicolumn{1}{l|}{ViT-Adapter-B} & 49.6 & 39.3 & 35.4 & 34.9 & 30.9 & 38.1 & 35.7 & 35.7 & 35.7 & 39.2 & 47.9 & 44.7 & 47.0 & 39.2 & 35.5 & 45.0 & 45.6 & 38.6 \\
                \rowcolor{yellow!20}
                \multicolumn{1}{l|}{ViT-Adapter-B$^\bigstar$} & \textbf{50.7} & \textbf{43.3} & 42.2 & 37.6 & 33.0 & 40.6 & 44.3 & 39.1 & 41.0 & 43.8 & 49.5 & 49.1 & 49.5 & 42.9 & 40.5 & 48.0 & 49.4 & 42.4 \\
                \midrule
                \multicolumn{1}{l|}{ViT-L$^*$~\cite{li2021benchmarking}} & 48.8 & 40.2 & 35.6 & 35.8 & 30.1 & 38.8 & 38.7 & 38.0 & 38.8 & 41.1 & 46.9 & 44.7 & 46.2 & 41.0 & 38.3 & 44.9 & 45.3 & 39.1 \\
                \rowcolor{gray!20}
                \multicolumn{1}{l|}{ViT-Adapter-L} & \textbf{50.9} & \textbf{42.3} & 37.3 & 37.1 & 30.2 & 40.5 & 41.1 & 41.0 & 41.1 & 43.4 & 49.5 & 47.7 & 48.5 & 42.9 & 39.7 & 47.1 & 48.4 & 41.4 \\
                \bottomrule
        \end{tabular}
        }
    }
    \end{center}
	
    \label{tab:robustness}
\end{table}

==> table/sota_city.tex <==

\begin{table}[t]\scriptsize
	\centering
	\caption{\textbf{Comparison with previous state-of-the-art results on the validation set and test set of Cityscapes.} 
	Here we load BEiT~\cite{bao2021beit} pre-trained weights to initialize our ViT-Adapter-L.
    ``MS" denotes multi-scale testing.
    ``Coarse" represents using extra 20k coarsely annotated images.
    }
    \setlength\tabcolsep{2.1mm}
    \begin{tabular}{l|cc|cc|cc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Coarse} & \multirow{2}{*}{Crop Size} & \multicolumn{2}{c|}{val set}  & \multicolumn{2}{c}{test set}\\
        & & & mIoU & +MS & mIoU & +MS\\
        \midrule
        SegFormer-B5~\cite{xie2021segformer} & \ding{55} & 1024$\times$1024 & 82.4 & 84.0 & - & 83.1 \\
        Swin-L  (Mask2Former)~\cite{liu2021swin} & \ding{55} & 512$\times$1024 & 83.3 & 84.3 & - & - \\
        SeMask-Swin-L  (Mask2Former)~\cite{jain2021semask} & \ding{55} & 512$\times$1024 & 84.0 & 85.0 & - & -  \\
        Lawin-Swin-L~\cite{jain2021semask} & \ding{55} & 1024$\times$1024 & - & - & - & 84.4  \\
        HRNet+OCR+SegFix~\cite{yuan2019segmentation} & $\checkmark$ & 769$\times$769 & - & - & 84.5 & -  \\
        HRNetV2+OCR+HMS~\cite{tao2020hierarchical} & $\checkmark$ & 1024$\times$2048 & \textbf{86.0} & \textbf{86.3} & - & 85.1  \\
        \midrule
	    \rowcolor{gray!20} 
        ViT-Adapter-L (Mask2Former) & \ding{55} & 896$\times$896 & 84.9 & 85.8 & - & \textbf{85.2} \\
	    \bottomrule
    \end{tabular}
    \label{tab:sota_city}
\end{table}

==> table/sota_cocostuff.tex <==
\begin{table}[t]\scriptsize
	\renewcommand{\arraystretch}{1.1}
	\caption{\textbf{Comparison with previous state-of-the-art results on COCO-Stuff-10K (left) and Pascal Context (right).} 
	Here we load BEiT~\cite{bao2021beit} pre-trained weights to initialize our ViT-Adapter-L.
    ``MS" denotes multi-scale testing.
    }
	\begin{minipage}{0.35\textwidth}%
	\centering
	\setlength\tabcolsep{1.2mm}
    \begin{tabular}{l|cc}
        \toprule
        Method & mIoU & +MS \\
	    \midrule
        %  EfficientNet-B7 (CAA)~\cite{huang2021channelized} & - & 45.4 \\
         ViT-L (StructToken-PWE)~\cite{lin2022structtoken} & - & 48.2 \\
         ViT-L (StructToken-CSE)~\cite{lin2022structtoken} & - & 48.7 \\
         ViT-L (StructToken-SSE)~\cite{lin2022structtoken} & - & 49.1 \\
         ConvNeXt-L+JPU (CAR)~\cite{huang2022car} & 49.0 & 50.0 \\ 
         Swin-L (SenFormer)~\cite{bousselham2021efficient} & 49.8 & 51.5 \\ 
         \midrule
         \rowcolor{gray!20}
         ViT-Adapter-L (UperNet) & 51.0 & 51.4 \\
         \rowcolor{gray!20}
         ViT-Adapter-L (Mask2Former) & \textbf{53.2} & \textbf{54.2} \\ 
	    \bottomrule
    \end{tabular}
    
    \end{minipage}
    \hspace{6.7em}
    \begin{minipage}{0.5\textwidth}%
    \setlength\tabcolsep{1.2mm}
    \begin{tabular}{l|cc}
        \toprule
        Method & mIoU & +MS \\
	    \midrule
	    ViT-L (SETR-MLA)~\cite{zheng2021rethinking} & - & 55.8 \\
	    ViT-L (Segmentor)~\cite{strudel2021segmenter} & - & 59.0 \\
	    ViT-Hybrid (DPT)~\cite{ranftl2021vision} & - & 60.5 \\
	   % EfficientNet-B7 (CAA)~\cite{huang2021channelized} & - & 60.5 \\
         ConvNeXt-L+JPU (CAR)~\cite{huang2022car} & 63.0 & 64.1 \\ 
         Swin-L (SenFormer)~\cite{bousselham2021efficient} & 63.1 & 64.5 \\ 
         \midrule
         \rowcolor{gray!20}
         ViT-Adapter-L (UperNet) & 67.0 & 67.5 \\ 
         \rowcolor{gray!20}
         ViT-Adapter-L (Mask2Former) & \textbf{67.8} & \textbf{68.2} \\ 
	    \bottomrule
    \end{tabular}
    \end{minipage}
    \label{tab:sota_cocostuff}
\end{table}
